Flux Rope Formation Due to Shearing and Zipper Reconnection

Zipper reconnection has been proposed as a mechanism for creating most of the twist in the flux tubes that are present prior to eruptive flares and coronal mass ejections. We have conducted a first numerical experiment on this new regime of reconnection, where two initially untwisted parallel flux tubes are sheared and reconnected to form a large flux rope. We describe the properties of this experiment, including the linkage of magnetic flux between concentrated flux sources at the base of the simulation, the twist of the newly formed flux rope and the conversion of mutual magnetic helicity in the sheared pre-reconnection state into the self-helicity of the newly formed flux rope.

==> math_def.tex <==
% This is my horrible mutated version of Claire Parnell's original math_def.tex file
% It hopefully contains lots of useful shortcuts, defined to make life easier..
% Oh and I stuck in some stuff from Bernie's analytical project too...


\newcommand{\diff}[2]{\frac{{\rm d}#1}{{\rm d}#2}}
\newcommand{\ndiff}[3]{\frac{{\rm d}^{#3}#1}{{\rm d}#2^{#3}}}
\newcommand{\pdiff}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\npdiff}[3]{\frac{\partial^{#3} #1}{\partial #2^{#3}}}
\newcommand{\e}[1]{\ensuremath{{\rm e}^{#1}}}
\newcommand{\ldiff}[2]{\ensuremath{{\rm d}#1/{\rm d}#2}}
\newcommand{\lpdiff}[2]{\ensuremath{\partial#1/\partial#2}}
\newcommand{\lnpdiff}[3]{\ensuremath{\partial^{#3}#1/\partial#2^{#3}}}

\newcommand{\vel}{ {\bf v} }
\newcommand{\Efi}{ {\bf E} }
\newcommand{\Bfi}{ {\bf B} }
\newcommand{\Afi}{ {\bf A} }
\newcommand{\rfi}{ {\bf r} }
\newcommand{\dipm}{ {\bf m} }
\newcommand{\Mag}{ {\bf M} }
\newcommand{\Hfi}{ {\bf H} }
\newcommand{\Dfi}{ {\bf D} }
\newcommand{\rvec}{ {\bf r} }
\newcommand{\Icur}{ {\bf I} }
\newcommand{\Kcur}{ {\bf K} }
\newcommand{\Jcur}{ {\bf J} }
\newcommand{\rvechat}{ {\bf{\hat r}} }
\newcommand{\ulin}{ \underline }
\newcommand{\beq}{ \begin{eqnarray} }
\newcommand{\eeq}{ \end{eqnarray} }
\newcommand{\dl}{ {\rm d}l }
\newcommand{\da}{ {\rm d}a }
\newcommand{\dt}{ {\rm d}\tau }
\newcommand{\bdl}{ {\bf{\rm d}l} }
\newcommand{\bda}{ {\bf{\rm d}a} }
\newcommand{\bdt}{ {\bf{\rm d}\tau} }
\newcommand{\nor}{ {\bf n} }
\newcommand{\rmd}{ {\rm d} }
\newcommand{\dR}{ {\rm d}R }
\newcommand{\dth}{ {\rm d}\theta }
\newcommand{\dphi}{ {\rm d}\phi }
\newcommand{\lra}{ \longrightarrow }
\newcommand{\Lra}{ \Longrightarrow }

\newcommand{\xhat}{ {{\bf{\hat x}}} }
\newcommand{\yhat}{ {{\bf{\hat y}}} }
\newcommand{\zhat}{ {{\bf{\hat z}}} }
\newcommand{\rhat}{ {\bf{\hat r}} }
\newcommand{\Rhat}{ {\bf{\hat R}} }
\newcommand{\that}{ {\boldsymbol{\hat \theta}} }
\newcommand{\phat}{ {\boldsymbol{\hat \phi}} }
\newcommand{\dive }{ {\bf {\nabla}} \cdot }
\newcommand{\curl }{ {\bf {\nabla}} \times }
\newcommand{\lap }{ {\bf\nabla}^2 }
\newcommand{\parx}{ {\partial x} }
\newcommand{\pary}{ {\partial y} }
\newcommand{\parz}{ {\parital z} }
\newcommand{\parR}{ {\partial R} }
\newcommand{\parp}{ {\partial \phi} }
\newcommand{\parr}{ {\partial r} }
\newcommand{\pt}{ {\partial \theta} }
\newcommand{\dxdt}{ \frac{dx}{dt} }
\newcommand{\dydt}{ \frac{dy}{dt} }
\newcommand{\dzdt}{ \frac{dz}{dt} }
\newcommand{\ddxdt}{ \frac{d^2x}{dt^2} }
\newcommand{\ddydt}{ \frac{d^2y}{dt^2} }
\newcommand{\ddzdt}{ \frac{d^2z}{dt^2} }
\newcommand{\dddxdt}{ \frac{d^3x}{dt^3} }
\newcommand{\dddydt}{ \frac{d^3y}{dt^3} }
\newcommand{\dddzdt}{ \frac{d^3z}{dt^3} }
\newcommand{\drdtl}{ {d\bf{r}}/{dt}  }
\newcommand{\drdt}{ \frac{d \bf{r}}{dt}  }
\newcommand{\ddrdt}{ \frac{d^2 \bf{r}}{dt^2}  }
\newcommand{\dddrdt}{ \frac{d^3 \bf{r}}{dt^3}  }
\newcommand{\vpar}{ v_{\parallel} }
\newcommand{\vperp}{ v_{\perp} }
\newcommand{\Eperp}{ E_{\perp} }
\newcommand{\Wpar}{ W_{\parallel} }
\newcommand{\Wperp}{ W_{\perp} }
\newcommand{\dvdt}{ \frac{d \bf{v}}{dt}  }
\newcommand{\dvxdt}{ \frac{dv_x}{dt} }
\newcommand{\dvydt}{ \frac{dv_y}{dt} }
\newcommand{\dvzdt}{ \frac{dv_z}{dt} }
\newcommand{\ddvxdt}{ \frac{d^2v_x}{dt^2} }
\newcommand{\ddvydt}{ \frac{d^2v_y}{dt^2} }
\newcommand{\ddvzdt}{ \frac{d^2v_z}{dt^2} }
\newcommand{\dvx}{ \.v_x }
\newcommand{\dvy}{ \.v_y }
\newcommand{\dvz}{ \.v_z }
\newcommand{\ddvx}{ \"v_x }
\newcommand{\ddvy}{ \"v_y }
\newcommand{\ddvz}{ \"v_z }
\newcommand{\dOdy}{ \frac{ d \Omega}{dy}}
\newcommand{\dOp}{ \Omega_{o}^{'} }
\newcommand{\dOyp}{ \Omega_{y}^{'} }
\newcommand{\ddvxpdt}{ \frac{d^2}{dt^2} \left( v_{x0} + v_{x1} \right) }
\newcommand{\ddvypdt}{  \frac{d^2}{dt^2} \left( v_{y0} + v_{y1} \right) }
\newcommand{\ddvxldt}{ \frac{d^2v_{x0}}{dt^2} }
\newcommand{\ddvyldt}{ \frac{d^2v_{y0}}{dt^2} }
\newcommand{\ddvxsdt}{ \frac{d^2v_{x1}}{dt^2} }
\newcommand{\ddvysdt}{ \frac{d^2v_{y1}}{dt^2} }
\newcommand{\vxp}{\left( v_{x0} + v_{x1} \right) }
\newcommand{\vyp}{\left( v_{y0} + v_{y1} \right) }

\newcommand{\boldnabla}{\mbox{\boldmath$\nabla$}}

%Definitions used by Roberts

\def\A{{Alfv\'en}}
\def\Amp{Amp\`ere}
\def\Aic{Alfv\'enic}
\def\eq{equation}
\def\eqs{equations }
\def\mhd{magnetohydrodynamic }
\def\mhds{magnetohydrodynamics }
\def\ma{magnetoacoustic }
\def\azimorder{\rm n}
\def\w{\omega}
\def\ww{\omega^2}
\def\cs{c_s}
\def\css{c_s^2}
\def\cse{c_{se}}
\def\csse{c_{se}^2}
\def\cc{c^2}
\def\ca{{c_A}}
\def\caa{c_A^2}
\def\cao{c_{A}}
\def\caao{c_{A}^2}
\def\co{c_{s}}
\def\coo{c_{s}^2}
\def\cf{c_f}
\def\cff{c_f^2}
\def\ct{c_t}
\def\ctt{c_t^2}
\def\cto{c_{t}}
\def\ctto{c_{t}^2}
\def\ck{c_k}
\def\ckk{c_k^2}
\def\ce{c_{se}}
\def\cee{c_{se}^2}
\def\cae{c_{Ae}}
\def\caae{c_{Ae}^2}
\def\cte{c_{te}}
\def\ctte{c_{te}^2}
\def\rhoo{{\rho}_{0}}
\def\rhoe{{\rho}_{e}}
\def\Bo{B_{0}}
\def\Boo{B_{0}^{2}}
\def\Be{B_{e}}
\def\kz{k_z}
\def\kzz{k_z^2}
\def\kk{k^2}
\def\kms{km s$^{-1}$}
\def\Ws{\Omega_{saus}}
\def\Wss{\Omega_{saus}^{2}}
\def\nus{\nu_{saus}}
\def\Ps{P_{saus}}
\def\Wk{\Omega_{k}}
\def\Wkk{\Omega_{k}^{2}}
\def\nuk{\nu_{k}}
\def\Pk{P_{k}}
\def\Wac{\Omega_{ac}}
\def\Wacc{\Omega_{ac}^{2}}
\def\WA{\Omega_{A}}
\def\WAA{\Omega_{A}^{2}}
\def\nuA{\nu_{A}}
\def\PA{P_{A}}

\def\grad{\boldnabla}

% My Own Personal Additions:
\def\eo{\epsilon_{0}}
\def\muo{\mu_{0}}
\def\kpar{{k_{\parallel}}}
\def\kper{{k_{\perp}}}
\def\vxx{{\bf{v}_x}}
\def\vyy{{\bf{v}_y}}
\def\vzz{{\bf{v}_z}}
\def\vx{v_x}
\def\vy{v_y}
\def\vz{v_z}
\def\xhat{\bf{\hat{x}}}
\def\yhat{\bf{\hat{y}}}
\def\zhat{\bf{\hat{z}}}
\def\vhat{\hat{v}}
\def\di{\delta_i}

\def\vscl{{v_{scl}}}
\def\vsclsq{{{v_{scl}}^2}}
\def\lscl{{l_{scl}}}
\def\tscl{{t_{scl}}}
\def\bscl{{b_{scl}}}
\def\escl{{{e_{scl}}}}
\def\enscl{{{en_{scl}}}}
\def\KEscl{{{{KE}_{scl}}}}
\def\omscl{{{\Omega_{scl}}}}
\def\muscl{{{\mu_{scl}}}}
%\def\vscl{{\color{OliveGreen}{v_{scl}}}}
%\def\vsclsq{{\color{OliveGreen}{{v_{scl}}^2}}}
%\def\lscl{{\color{OliveGreen}{l_{scl}}}}
%\def\tscl{{\color{OliveGreen}{t_{scl}}}}
%\def\bscl{{\color{OliveGreen}{b_{scl}}}}
%\def\escl{{\color{OliveGreen}{e_{scl}}}}
%\def\enscl{{\color{OliveGreen}{en_{scl}}}}
%\def\omscl{{\color{OliveGreen}{\Omega_{e}^{scl}}}}
%\def\muscl{{\color{OliveGreen}{\mu_{scl}}}}

\newcommand{\angstrom}{\mbox{\normalfont\AA}}
\newcommand{\Epar}{E_{\parallel}}
\newcommand{\upar}{u_{\parallel}}
\newcommand{\ue}{{{\bf{u}}_E}}
\newcommand{\ugb}{{\bf{u}}_{\grad{B}}}
%\def\o{c_{A0}}
%\def\caao{c_{A0}^2}
%\def\co{c_{0}}
%\def\coo{c_{0}^2}
%\def\cto{c_{t0}}
%\def\ctto{c_{t0}^2}
%EndDefinitions

